Bayesian Target-Vector Optimization for Efficient Parameter Reconstruction

Parameter reconstructions are indispensable in metrology. Here, the objective is to to explain $K$ experimental measurements by fitting to them a parameterized model of the measurement process. The model parameters are regularly determined by least-square methods, i.e., by minimizing the sum of the squared residuals between the $K$ model predictions and the $K$ experimental observations, $\chi^2$. The model functions often involve computationally demanding numerical simulations. Bayesian optimization methods are specifically suited for minimizing expensive model functions. However, in contrast to least-square methods such as the Levenberg-Marquardt algorithm, they only take the value of $\chi^2$ into account, and neglect the $K$ individual model outputs. We present a Bayesian target-vector optimization scheme with improved performance over previous developments, that considers all $K$ contributions of the model function and that is specifically suited for parameter reconstruction problems which are often based on hundreds of observations. Its performance is compared to established methods for an optical metrology reconstruction problem and two synthetic least-squares problems. The proposed method outperforms established optimization methods. It also enables to determine accurate uncertainty estimates with very few observations of the actual model function by using Markov chain Monte Carlo sampling on a trained surrogate model.

==> Makefile <==
MAIN=paper
SOURCES=$(MAIN).tex Makefile

LATEX=pdflatex
LATEXOPT=-shell-escape
NONSTOP=-interaction nonstopmode

LATEXMK=latexmk
LATEXMKOPT=-pdf
CONTINUOUS=-pvc
FORCE=-f

all:    $(MAIN).pdf

.refresh:
	touch .refresh

$(MAIN).pdf: $(MAIN).tex .refresh $(SOURCES)
	$(LATEXMK) $(LATEXMKOPT) \
	-pdflatex="$(LATEX) $(LATEXOPT) $(NONSTOP) %O %S" $(MAIN)

supplement: supplement.tex .refresh
	$(LATEXMK) $(LATEXMKOPT) \
	-pdflatex="$(LATEX) $(LATEXOPT) $(NONSTOP) %O %S" supplement


force:
	touch .refresh
	rm -f $(MAIN).pdf
	$(LATEXMK) $(LATEXMKOPT) $(FORCE) \
	-pdflatex="$(LATEX) $(LATEXOPT) %O %S" $(MAIN)

clean:
	$(LATEXMK) -c $(MAIN)
	rm -f $(MAIN).pdfsync
	rm -rf *~ *.tmp
	rm -f *.blg *.aux *.end *.fls *.log *.out *.fdb_latexmk
	rm -f *.xml .refresh *-blx.*
	rm -rf *.acn *.acr *.acrLOG *.glo *.ist
	rm -rf *.auxlock
	rm -rf *.gls
	rm -rf *.glsLOG
	rm -rf $(MAIN)-figure*
	rm -rf *.script
	rm -rf auto/
	rm -rf tikzcache/*

deepclean: clean
	rm -f paper.pdf
	rm -f supplement.pdf

once:
	$(LATEXMK) $(LATEXMKOPT) -pdflatex="$(LATEX) $(LATEXOPT) %O %S" $(MAIN)

continuous: $(MAIN).tex .refresh $(SOURCES)
	$(LATEXMK) $(LATEXMKOPT) $(CONTINUOUS) \
	-pdflatex="$(LATEX) $(LATEXOPT) $(NONSTOP) %O %S" $(MAIN)

debug:
	$(LATEX) $(LATEXOPT) $(MAIN)

.PHONY: clean force once all

